Are Easy Data Easy (for K-Means)

This paper investigates the capability of correctly recovering well-separated clusters by various brands of the $k$-means algorithm. The concept of well-separatedness used here is derived directly from the common definition of clusters, which imposes an interplay between the requirements of within-cluster-homogenicity and between-clusters-diversity. Conditions are derived for a special case of well-separated clusters such that the global minimum of $k$-means cost function coincides with the well-separatedness. An experimental investigation is performed to find out whether or no various brands of $k$-means are actually capable of discovering well separated clusters. It turns out that they are not. A new algorithm is proposed that is a variation of $k$-means++ via repeated {sub}sampling when choosing a seed. The new algorithm outperforms four other algorithms from $k$-means family on the task.

==> PDFS/worst_mdKmeans_8-8-30-10-40-40.tex <==


\begin{figure}
\begin{center}
\includegraphics[width=0.49\textwidth]{ PDFS/worst_mdKmeans_8_8_30_10_40_40.pdf } % 
\end{center}
\caption{Worst misclustering errors
 \mdKmeans {} 
 for the number of clusters $k$= 8 x 8 = 64  
noise level= 30 \%, cluster radius= 10 , cluster size= 40 , 
motion freedom of clusters= 40 , 
minimal distance between clusters: 5.83 *R} \label{fig:mdKmeans-8-8-30-10-40-40} 
 \end{figure}


==> PDFS/worst_mdKmeans_8-8-30-10-96-10.tex <==


\begin{figure}
\begin{center}
\includegraphics[width=0.49\textwidth]{ PDFS/worst_mdKmeans_8_8_30_10_96_10.pdf } % 
\end{center}
\caption{Worst misclustering errors
 \mdKmeans {} 
 for the number of clusters $k$= 8 x 8 = 64  
noise level= 30 \%, cluster radius= 10 , cluster size= 96 , 
motion freedom of clusters= 10 , 
minimal distance between clusters: 5.83 *R} \label{fig:mdKmeans-8-8-30-10-96-10} 
 \end{figure}


==> PDFS/worst_pbKmeans_8-8-30-10-96-10.tex <==


\begin{figure}
\begin{center}
\includegraphics[width=0.49\textwidth]{ PDFS/worst_pbKmeans_8_8_30_10_96_10.pdf } % 
\end{center}
\caption{Worst misclustering errors
 \pbKmeans {} 
 for the number of clusters $k$= 8 x 8 = 64  
noise level= 30 \%, cluster radius= 10 , cluster size= 96 , 
motion freedom of clusters= 10 , 
minimal distance between clusters: 5.83 *R} \label{fig:pbKmeans-8-8-30-10-96-10} 
 \end{figure}


==> PDFS/worst_tcKmeans_8-8-30-10-96-10.tex <==


\begin{figure}
\begin{center}
\includegraphics[width=0.49\textwidth]{ PDFS/worst_tcKmeans_8_8_30_10_96_10.pdf } % 
\end{center}
\caption{Worst misclustering errors
 \tcKmeans {} 
 for the number of clusters $k$= 8 x 8 = 64  
noise level= 30 \%, cluster radius= 10 , cluster size= 96 , 
motion freedom of clusters= 10 , 
minimal distance between clusters: 5.83 *R} \label{fig:tcKmeans-8-8-30-10-96-10} 
 \end{figure}

